Political Polarization in Online News Consumption

Political polarization appears to be on the rise, as measured by voting behavior, general affect towards opposing partisans and their parties, and contents posted and consumed online. Research over the years has focused on the role of the Web as a driver of polarization. In order to further our understanding of the factors behind online polarization, in the present work we collect and analyze Web browsing histories of tens of thousands of users alongside careful measurements of the time spent browsing various news sources. We show that online news consumption follows a polarized pattern, where users' visits to news sources aligned with their own political leaning are substantially longer than their visits to other news sources. Next, we show that such preferences hold at the individual as well as the population level, as evidenced by the emergence of clear partisan communities of news domains from aggregated browsing patterns. Finally, we tackle the important question of the role of user choices in polarization. Are users simply following the links proffered by their Web environment, or do they exacerbate partisan polarization by intentionally pursuing like-minded news sources? To answer this question, we compare browsing patterns with the underlying hyperlink structure spanned by the considered news domains, finding strong evidence of polarization in partisan browsing habits beyond that which can be explained by the hyperlink structure of the Web.

==> 006social_media.tex <==
\subsection{Twitter users}

I also checked the number of users for whom we can get the Twitter account from their browse logs. It was not easy to get, but using the four methods below, I was able to get the twitter username for over 600 out of the 3942 political users (users who had visited at least 50 visits to a political website).
Users visiting analytics.twitter.com which takes them to a url specific to their username, (25\%)
Users tweeting something, which reveals the tweet id of the tweet. We can get the username by looking up the author of the tweetid. (60\%)
Users reporting other users/tweets reveals their user id. (5\%)
Users who tried to login but entered their password wrong (10\%).

We computed the polarity scores of users according to various external metrics including Barbera et al.\cite{barbera2015birds} and Garimella et al.~\cite{garimella2018political}. 

We find that the consumption as evidenced on our platform and production scores are correlated.

Figure~\ref{fig:production_barbera} shows the consumption polarity obtained from pioneer to leaning scores obtained from Barbera et al.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth, height=0.5\textwidth]{images/twitter1.png}
    \caption{Correlation between pioneer consumption polarity and Barbera et al.}
    \label{fig:production_barbera}
\end{figure}

Figure~\ref{fig:production_pioneer_garimella} shows the correlation between consumption on pioneer and production on twitter.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth, height=0.5\textwidth]{images/twitter2.png}
    \caption{Comparison between pioneer consumption polarity and production polarity on twitter.}
    \label{fig:production_pioneer_garimella}
\end{figure}




==> macros.tex <==
% !TEX root =  qscore.tex

% Packages
\usepackage{type1cm}     % type1 computer modern font
\usepackage{graphicx}     % advanced figures
\usepackage{xspace}     % fix space in macros
%\usepackage{balance}     % to better equalize the last page
\usepackage{booktabs}     % nicer tables
\usepackage{multirow}      % multirow for tables
%\usepackage[tableposition=top]{caption}     % captions on top for tables
% \usepackage[hyphens]{url}     % handle long urls
% \usepackage{bold-extra}     % bold + {small capital, italic}
% \usepackage{siunitx}          % \num for decimal grouping
\usepackage[vlined,linesnumbered,ruled,noend]{algorithm2e}     % algorithms
%\usepackage{natbib}     % better references
\usepackage{microtype}    % compress text
\usepackage{units}     % nicer slanted fractions
\usepackage{mathtools}     % amsmath++
\usepackage{amsmath}
\usepackage{amssymb}     % math symbols
\usepackage{xfrac}    % sfrac
\usepackage[font={small}]{subfig} % subfig, 4 figures in a row
%\usepackage{float}
\usepackage[show]{chato-notes}
\usepackage{enumitem}
\usepackage{makecell}
%\usepackage{subcaption}
%\usepackage{flushend}
\usepackage{mathtools,xparse}

% Hyperref is forbidden (it also screws up the bibliography):
% https://www.aaai.org/Publications/Author/formatting-instructions-latex.pdf
% \usepackage[draft]{hyperref}
% \usepackage[bookmarks, pdftex, colorlinks=false]{hyperref}     % clickable references

%\usepackage[T1]{fontenc} %to solve the font error
%\usepackage{lipsum} %to solve the font error
\usepackage{hyphenat}


%\setcounter{tocdepth}{3}
\graphicspath{{img/}}

% Bibliography
% \setlength{\bibsep}{1pt}
% \renewcommand{\bibfont}{\small\raggedright}
% \renewcommand{\bibsection}{\section{REFERENCES}\vspace{-.5\baselineskip}}

%% notation
\newcommand{\usergraph}{\ensuremath{G}\xspace}
\newcommand{\users}{\ensuremath{U}\xspace}
\newcommand{\user}{\ensuremath{u}\xspace}
\newcommand{\edges}{\ensuremath{E}\xspace}
\newcommand{\edge}{\ensuremath{e}\xspace}
\newcommand{\edgeweight}{\ensuremath{w}\xspace}
\newcommand{\nousers}{\ensuremath{n}\xspace}
\newcommand{\sources}{\ensuremath{S}\xspace}
\newcommand{\source}{\ensuremath{s}\xspace}
\newcommand{\nosources}{\ensuremath{m}\xspace}
\newcommand{\noclusters}{\ensuremath{k}\xspace}
\newcommand{\ideology}{\ensuremath{i}\xspace}
% U : users
% S : sources
% C : clusters
% L : laplacian
\newcommand{\UUmat}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\USmat}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\UCmat}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\SCmat}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\CCUmat}{\ensuremath{\mathbf{H}_u}\xspace}
\newcommand{\CCSmat}{\ensuremath{\mathbf{H}_s}\xspace}
\newcommand{\ULmat}{\ensuremath{\mathbf{L}_u}\xspace}
\newcommand{\VLmat}{\ensuremath{\mathbf{L}_v}\xspace}
\newcommand{\SLmat}{\ensuremath{\mathbf{L}_s}\xspace}
\newcommand{\WLmat}{\ensuremath{\mathbf{L}_w}\xspace}
\newcommand{\ZLmat}{\ensuremath{\mathbf{L}_z}\xspace}
\newcommand{\regparamone}{\ensuremath{\alpha}\xspace}
\newcommand{\regparamtwo}{\ensuremath{\beta}\xspace}
\newcommand{\trace}[1]{\ensuremath{\mathit{tr}({#1})}\xspace}
% other matrices, to be used as variables
\newcommand{\Dmat}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\Xmat}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\Wmat}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\Hmat}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\Zmat}{\ensuremath{\mathbf{Z}}\xspace}
\newcommand{\Umat}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\Lmat}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\eye}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\xrow}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\urow}{\ensuremath{\mathbf{u}}\xspace}
%% some more variables for users and objects
\newcommand{\usera}{\ensuremath{u}\xspace}
\newcommand{\userb}{\ensuremath{v}\xspace}
\newcommand{\userc}{\ensuremath{w}\xspace}
\newcommand{\useri}{\ensuremath{u_i}\xspace}
\newcommand{\userj}{\ensuremath{u_j}\xspace}
\newcommand{\userk}{\ensuremath{u_k}\xspace}
\newcommand{\obji}{\ensuremath{o_i}\xspace}
\newcommand{\objj}{\ensuremath{o_j}\xspace}
\newcommand{\objk}{\ensuremath{o_k}\xspace}
\newcommand{\objects}{\ensuremath{O}\xspace}
%
\newcommand{\rown}[1]{\ensuremath{{#1}_{\mathit{rn}}}\xspace}
\newcommand{\coln}[1]{\ensuremath{{#1}_{\mathit{cn}}}\xspace}
% \newcommand{\rown}[1]{\ensuremath{\mathit{rn}({#1})}\xspace}
% \newcommand{\coln}[1]{\ensuremath{\mathit{cn}({#1})}\xspace}
\newcommand{\xcoord}{\ensuremath{x}\xspace}
\newcommand{\ycoord}{\ensuremath{y}\xspace}
\newcommand{\iscore}[2]{\ensuremath{i({#1},{#2})}\xspace}
\newcommand{\popscore}[2]{\ensuremath{\rho({#1},{#2})}\xspace}


\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\normOne}{\left|}{\right|}
\DeclarePairedDelimiter{\vectorBrackets}{\langle}{\rangle}

\NewDocumentCommand{\normL}{ s O{} m }{%
    \IfBooleanTF{#1}{\norm*{#3}}{\norm[#2]{#3}}_{F}^2%
}
\NewDocumentCommand{\normF}{ s O{} m }{%
     \IfBooleanTF{#1}{\norm*{#3}}{\norm[#2]{#3}}_{F}%
}
\NewDocumentCommand{\normsquare}{ s O{} m }{%
    \IfBooleanTF{#1}{\norm*{#3}}{\norm[#2]{#3}}^2%
}

\newcommand{\reals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\nmf}{{\sc\Large nmf}\xspace}
\newcommand{\NMFSymm}{{\sc\Large nmf-symm}\xspace}
\newcommand{\onmft}{{\sc\Large onmtf}\xspace}
\newcommand{\dmcc}{{\sc\Large dmcc}\xspace}
\newcommand{\prob}{{\sc\Large ifd}\xspace}
\newcommand{\probngr}{{\sc\Large ifd-ngr}\xspace}
\newcommand{\purity}{{\sc\Large purity}\xspace}
\newcommand{\AMI}{{\sc\Large ami}\xspace}
\newcommand{\NMI}{{\sc\Large nmi}\xspace}
\newcommand{\ARI}{{\sc\Large ari}\xspace}
\newcommand{\PMCC}{{\sc\Large corr}\xspace}
\newcommand{\PMCCi}{{\sc\Large corr$_i$}\xspace}
\newcommand{\PMCCp}{{\sc\Large corr$_\rho$}\xspace}
\newcommand{\retweet}{{\sc\Large retweet}\xspace}
\newcommand{\follow}{{\sc\Large follow}\xspace}
\newcommand{\avgcontent}{{\sc\Large avg\_content}\xspace}
\newcommand{\content}{{\sc\Large content}\xspace}

\DeclareMathOperator{\idf}{idf}
\DeclareMathOperator{\tf}{tf}
\newcommand{\tfidf}{\ensuremath{\tf \cdot \idf}\xspace}

% Bibliography
%\setlength{\bibsep}{1pt}
%\renewcommand{\bibfont}{\small\raggedright}
%\renewcommand{\bibsection}{\section{References}\vspace{-.5\baselineskip}}

% Paragraphs
\newcommand{\spara}[1]{\smallskip\noindent\textbf{#1.}}
\newcommand{\sparaNoPeriod}[1]{\smallskip\noindent\textbf{#1}}
\newcommand{\mpara}[1]{\medskip\noindent\textbf{#1}}
\newcommand{\para}[1]{\noindent\textbf{#1}}

%datasets
\newcommand{\cpt}[1]{\textsc{\MakeLowercase{#1}}}
\newcommand{\verified}{\cpt{Verified}\xspace}
\newcommand{\political}{\cpt{Political}\xspace}
\newcommand{\despoina}{\cpt{Despoina}\xspace}
\newcommand{\despoinarandom}{\cpt{Despoina (random)}\xspace}
\newcommand{\instagram}{\cpt{Instagram}\xspace}
\newcommand{\youtube}{\cpt{YouTube}\xspace}
\newcommand{\mrt}{\textsc{MRT}\xspace}
\newcommand{\nmrt}{\textsc{NMRT}\xspace}

%% definitions
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{observation}{Observation}
\newtheorem{problem}{Problem}
\newtheorem{thm}{Theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{property}{Property}
%\newtheorem{proof}{Proof}
%\newtheorem{corollary}{Corollary}
%\newtheorem{example}{Example}


% Squishlist
\newenvironment{squishlist}
{\begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{1pt}
     \setlength{\topsep}{1pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
{\end{list}}

\newcommand{\Diff}{\mathrm{d}}
\newcommand{\tmin}{\epsilon}

\newcommand{\hide}[1]{}

\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1.}}}
\newcommand{\xhdrNoPeriod}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}

% References for sections and tables:
\newcommand{\Secref}[1]{Sec.~\ref{#1}}
\newcommand{\Eqnref}[1]{Eq.~\ref{#1}}
\newcommand{\Dashsecref}[2]{Sec.~\ref{#1}--\ref{#2}}
\newcommand{\Dblsecref}[2]{Sec.~\ref{#1} and \ref{#2}}
\newcommand{\Tabref}[1]{Table~\ref{#1}}
\newcommand{\Figref}[1]{Fig.~\ref{#1}}
\newcommand{\Dashfigref}[2]{Fig.~\ref{#1}--\ref{#2}}
\newcommand{\Appref}[1]{Appendix~\ref{#1}}


\newcommand{\ie}{{i.e.}\xspace}
\newcommand{\eg}{{e.g.}\xspace}
\newcommand{\cf}{{cf.}\xspace}
\newcommand{\etal}{{et al.}\xspace}
\newcommand{\vs}{{vs.}\xspace}
\newcommand{\etc}{{etc.}\xspace}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\cmarkbold}{\ding{52}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\xmarkbold}{\ding{56}}

\newcommand{\textcite}[1]{\citeauthor{#1} \shortcite{#1}}

% Bob's package for nice Greek letters within a Times math environment.
\usepackage{cmm-greek}

% to get formulae in the time font as well:
\usepackage{mathptmx}


\clubpenalty = 10000
\widowpenalty = 10000 

